A Survey of Recent Advances and Challenges in Deep Audio-Visual Correlation Learning

Audio-visual correlation learning aims to capture and understand natural phenomena between audio and visual data. The rapid growth of Deep Learning propelled the development of proposals that process audio-visual data and can be observed in the number of proposals in the past years. Thus encouraging the development of a comprehensive survey. Besides analyzing the models used in this context, we also discuss some tasks of definition and paradigm applied in AI multimedia. In addition, we investigate objective functions frequently used and discuss how audio-visual data is exploited in the optimization process, i.e., the different methodologies for representing knowledge in the audio-visual domain. In fact, we focus on how human-understandable mechanisms, i.e., structured knowledge that reflects comprehensible knowledge, can guide the learning process. Most importantly, we provide a summarization of the recent progress of Audio-Visual Correlation Learning (AVCL) and discuss the future research directions.

==> sections/conclusion_task.tex <==
\section{Conclusion per task}
\label{appendix:conclusion-tasks}

% Generation
For generation (between modalities), we observed that most approaches rely on \acrshort*{gan}s and \acrshort*{ae}s. Both allow the generation of samples from one modality using the other, but \acrshort*{gan}s allow to generate new samples (i.e., not existing in the training set) and to obtain better performances in reconstruction. At the same time, we have seen many proposals that leverage \acrshort*{ae}s to condition in the generator's reconstruction and the discriminator's decision \cite{fanzeres2021sound}. We have seen the promising results the transformer architecture provides for translation/generation of sequence-based data (e.g., MIDI) \cite{gan2020foley}. We believe that the field can benefit from more research into dynamic pooling processes, i.e. attention, that allow the pooling of information from multiple modalities while balancing the amount of information extracted from each one. We argue that such research can enable new attention-based architectures that allow to condition the generation of new samples from multiple modalities. For other types of \acrshort*{av} data \acrshort*{cnn}-based approaches like \acrshort*{ae}s and their extensions are preferred for being used with matrix-like data (e.g., spectrograms, images).\par

% Recognition
Recognition proposals comprise self-supervised methods for \acrshort*{avcl}, evaluated in other downstream tasks. Typically, to evaluate their models, the authors fine-tune a linear classifier with the representations extracted with them. Self-supervised learning methods allow to obtain better performances than supervised ones. We observed that these methods already have tried to gather positive and negative samples from media at different framerates \cite{recasens2021broaden}, from the same temporal window (i.e., assuming that it contains the same context) \cite{recasens2021broaden}, and their augmented versions \cite{patrick2020multi}. According to this idea, the field could benefit from analysing how sampling can be made for the different modalities (i.e., audio and video channels) and how those methods allow to infer the ``context'' of a given audio and visual event. We leave this study for future work.\par

% Retrieval
Retrieval comprises all the methods used to search for similar items within the same modality or in others (if the dataset contains paired data). Results are reported in annotated datasets using supervised solutions. However, it does not imply that self-supervised approaches in zero-shot settings. We expect the field to progress toward those self-supervised methods due to their promising performances \cite{afouras2021self,rouditchenko2020avlnet}. Our research identified that most retrieval methods are built with methods that include loss functions with several linear components. Hence, the different regularisation methods are presented in Table \ref{tab:methods-final}. Each tackles a different desired aspect of the embedding space (i.e., representation space where retrieval is performed). This joint optimisation scheme typically maximises the alignment/correlation between modalities while minimising intra-class dispersion and maximising inter-class distances. We observed a progressive adoption of attention mechanisms and \acrshort*{ae}s for alignment of latent spaces and dimensionality reduction, respectively, which allowed us to increase the retrieval performances \cite{wu2019unified,rouditchenko2020avlnet}. Similarly to the previous applications, we also expect to see increasing adoption of self-supervised learning paradigms for retrieval.\par

% Sound localisation and separation
As the name suggests, sound localisation and separation consist of locating sound sources in the video feed and separating them in the audio clip. In localisation, spatial attention is the most used methodology to correlate sound sources to locations in the feature maps extracted by \acrshort*{cnn}s \cite{lin2021exploiting} and has shown good performances. Progressively, we have seen the proposal of self-supervised mixed with sampling approaches for visual patches and audio segments \cite{morgado2020learning,localiVisSounds}. Proposals typically leverage supervised datasets composed of audio spectrum with overlapping and separated sound sources for sound separation. Thus, results are commonly reported using reconstruction metrics for audio spectrums (e.g., \acrfull*{sdr}). Here, proposals based on \acrshort*{ae}s allow us to obtain the best performances. Methods that use different visual features (e.g., optical flow and \acrshort*{cnn}-based \cite{gao2019co,zhao2019sound}) are the ones to obtain the lowest \acrshort*{sdr}. Thus, the visual modality might be further explored to learn how to separate audio sources better.\par

==> sections/prob-def.tex <==
\section{Problem Definition}
\label{section:problem-definition}

Data is provided as tuples of arbitrary sizes.
$$
{x^{(n)} = (x_a^n, x_v^n)}_{n=1}^N \\
%{x_{a}} \in {\mathbb{R}^{d_{a}}} \\
%{x_{v}} \in {\mathbb{R}^{d_{v}}} \\
$$

The problem of Deep \acrshort*{avcl} can be formulated as follows. We are interested in data consisting of tuples ${x^{(n)} = (x_a^n, x_v^n)}_{n=1}^N$, where $x_a$ and $x_v$ are features extracted for audio and visual data respectively. These ``features'' can have multiple dimensions, they can be represented as vectors or (feature) maps. Therefore, for the purpose of our study, we consider them to be the same, we view them as encoded modalities. Both representations belong to separate sub-spaces and can have different dimensions, thus we represent them as ${x_{a}} \in {\mathbb{R}^{d_{a}}}$ and $x_v \in \mathbb{R}^{d_v}$ for audio and visual data respectively, where $d_{a}$ and $d_{v}$ can have 1 or more dimensions.\par

\acrshort*{avcl} seeks to project both audio and visual data through \acrfull*{dnn} into their own feature sub-spaces where the joint space composed by their aggregation preserves the shared information contained in each modality. That is to say, representations are bridged/related in a common space $S$ through $f(x_a;W_{a})$ and $g(x_v;W_{v})$, which respectively provide the sub-spaces $S_{\text{audio}}$ and $S_{\text{video}}$. The weights of $f$ and $g$ are adjusted through back-propagation in order to maximize the correlation between audio and visual data. The ``joint'' space from this process can be obtained through feature fusion or coordination, where the final output consists of single or parallel representations respectively.\par

This learning problem can be established as a supervised, self-supervised or unsupervised task depending on how relations between modalities are used. For instance, exploring relations within tuples $(x_{a}^{n_1}, x_{v}^{n_2})_{n_1 = n_2}$ and assuming each pair as having specific semantics allows to extract correlations in a self-supervised way. In contrast, it can also be desirable to relate modalities as a whole $(x_{a}^{n_1}, x_{v}^{n_2})_{n_1 = n_2 \vee n_1 \neq n_2}$ and take into account supervised information (i.e., labels) regarding each tuple.\par

==> tables/applications-table.tex <==
{
\scriptsize
\begin{longtable}{p{0.05\linewidth}p{0.9\linewidth}}
    \caption{Overview of specific application scenarios of representative works for audio-visual correlation learning}
    \label{tab:applications-final}\\
    \hline
    Paper & What was explored? \\ \hline
    \endfirsthead
    %
    \endhead
    %
    \hline
    \endfoot
    %
    \endlastfoot
    %
    \cite{mohamed2022learning}              & Applied a hierarchical Transformer model using concatenated inputs (from audio and visual data). The model was trained with masked sequence learning, where the goal is to predict the masked embeddings (for each modality). The model learns to use the global context from concatenated modalities. \\ %new
    \cite{chen2021vset}                     & Applied a multimodal transformer (co/cross-attention) in which audio is used to query visual data. The model was trained to generate a clean speech version of the original audio. The model was trained to reconstruct the original input, but was evaluated using the ratio of Power Spectra between clean and noisy speech. \\ %new
    \cite{sadeghi2019audio}                 & Applied a probabilistic latent model (VAE) over concatenated audio and visual embeddings from videos to produce a clean speech version of the original audio.\\ %new
    \cite{zhu2022discrete}                  & Applied a VQ-based encoder-decoder model based in the diffusion process. The model learns to reconstruct audio conditioned on the visual input.\\ %new
    \cite{fanzeres2021sound}                & Applied a GAN model in which the generator was a U-Net model that uses audio to reconstruct images. The latent representation from the Generator (autoencoder inspired by DenseNet) is used to condition the discriminator's decision (concatenation with the FC layer from the discriminator).\\
    \cite{zhu2021learning}                  & Applied VAEs to generate audio using visual data (video) and vice-versa. The Adv. Loss was used in this scenario to reduce the heterogeneity gap between modalities. The authors also proposed to include the Wasserstein loss as regularization term to improve alignment between representations.\\
    \cite{mira2021end}                      & Applied an \acrshort*{ae} model with different loss terms that considered different aspects of spectrograms (e.g., power, frequency and perceptual quality). \\
    \cite{gan2020foley}                     & Applied a Transformer model to translate between keypoints extracted from videos of people playing instruments and MIDI output (music). \\
    \cite{zhu2022quantized}                 & Applied a \acrshort*{gan} model to generate audio samples conditioned on visual inputs composed of concatenated motion and visual features. The goal is to receive human body motions and visual frames as input, and generate music according to the inputs. The generation of audio is made using VQ-based representations.\\%new
    \hline
    \cite{rajan2021robust}                  & Applied parallel \acrshort*{ae}s to reconstruct both modalities. Both latent spaces were conditioned using an additional loss term, which constrained them to be aligned.\\
    \cite{wu2021exploring}                  & Applied parallel projectors and constrained them to be correlated using co/cross-attention. The authors propose to exchange corresponding modalities during training and learned representations by contrasting temporal segments (Contrastive Learning). \\%new
    \cite{seo2020hmtl}                      & Applied parallel models for sentiment classification using large models for textual classification and a smaller attention-based model using audio and visual inputs. The goal is to use Adversarial Learning to reduce the gap between modalities and knowledge transfer to provide semantic information to the smaller model.\\
    \cite{zhang2019deep}                    & Applied co/cross-attention between audio and visual data for emotion recognition. The model used uni-modal self-attention and bilinear pooling to correlate visual facial features and speech.\\
    \cite{sun2023masked}                    & Applied the VideoMAE architecture for reconstructing motion from the original video input. The model is trained by predicting the content of the masked regions, i.e. motion trajectory containing position changes and shape change of moving objects.\\%new
    \cite{alwassel2019self}                 & Applied parallel projectors to create multimodal embeddings. The audio and visual features are concatenated and clustered using k-means to produce pseudo-labels to train the projectors.\\%new
    \cite{patrick2020multi}                 & Applied parallel encoders for audio and visual data to different segments of the original video (timesteps). The authors proposed a self-supervised framework that explored relations between different video frame sequences and segments within each video (temporal shifts and augmentation) to learn AV representations.\\
    \cite{sarkar2022xkd}                    & Applied masked reconstruction of parallel modalities. The reconstructions were aligned using the mean discrepancy between latent spaces. Knowledge from this larger \acrshort*{ae} model is transferred to a smaller one using KD.\\%new
    \cite{ma2020active}                     & Applied active learning in self-supervised learning paradigms to select negative samples. Parallel projectors were trained using contrastive losses.\\
    \cite{recasens2021broaden}              & Applied \acrshort*{ae}s to reconstruct between broader/narrower temporal views with high/low resolution from the same video frame sequence. Knowledge was given to the model using the same video clip with different resolutions, i.e. different dimensions.\\
    \cite{mm-versatile2020}                 & Applied parallel projections between three modalities: text, audio and visual data. The latent representations were aligned using self-supervised learning frameworks that use the temporal co-occurrence between audio-visual and textual-visual pairs.\\
    \cite{min2021cross}                     & Applied parallel projectors and co/cross-attention between feature extractors (using conv. filters) at different scales for aligning different modalities. \\
    \cite{akbari2021vatt}                   & Applied self-supervised learning frameworks to obtain a single joint space composed by separate common spaces (audio-video and video-text). Similar to \cite{mm-versatile2020}.\\
    \cite{cheng2020look}                    & Applied co/cross-attention between Transformer encoders by exchanging the query embedding between modalities. The authors benchmarked different attention methods (using Transformers) for multimodal alignment (i.e., synchronization). Their goal is to synchronize both modalities by predicting if they are synchronized or not (binary classification).\\
    \cite{qian2022multimodal}               & Applied cross-attention between audio and visual data (RGB + Flow). It starts by applying the same encoder for each modality. Temporal cohesion is ensured for the visual modality by using self-attention to learn relations between frames. Multimodal correlation is explored through cross-attention between modalities. It introduced semantic context using a frozen language/text encoder.\\%new
    \cite{sarkar2021self}                   & Applied a self-supervised framework for learning multimodal representations from audio segments. It leverages the cosine distance between embeddings between synchronized and non-synchronized segments. The non-synchronized (asynchronous) component aims to exploit the relationship between AV segments sampled at different timestamps.\\%new
    \cite{xuan2021discriminative}           & Proposed an extension of Deep Cluster CCA. Combination of spatial, temporal, and attention between modalities. Audio and visual data are fused using attention and coordinated using a loss function based on distances between elements. It projects both attended representations (A and V) to a common discriminative representation space. It considers inter and intra-modal info. The model follows eigenvalue-based learning scheme.\\%new
    \cite{gan2020cross}                     & Applied a co/cross-attention model between parallel modalities for video event location. The co/cross-attention module included channel and spatial wise summation of features between both modalities.\\ %new
    \cite{lee2021crossattentional}          & Applied multi-stage co/cross-attention between parallel modalities. The model was trained for classification using an open-max classifier (without knowing the whole set of classes), which takes the concatenated audio-visual features as input and generates classification scores for action classes and background.\\%new
    \cite{yang2019dual}                     & Applied co/cross-attention to filter relevant features for each modality by taking into account the other one. The authors' goal is to use the co/cross-attention mechanism to model the relation between the global features of one modality and the local features of the other. Global features are extracted for the whole video frame sequence, while local features only contain the relevant event. The approach is based on the idea that information is different between event and background segments.\\%new
    \cite{huang2022mavil}                   & Applied Proposed to learn AV representations using 3 forms of self-supervision that explore intra and inter-relationships between modalities. Afterwards, to obtain a homogeneous representation space, the authors implemented a masked prediction learning strategy that focuses on predicting missing portions of audio and visual inputs.\\%new
    \cite{arnab2022audiovisual}             & Applied a masked \acrshort*{ae}, to learn multimodal representations. Both modalities share the decoder and encoders' weights.\\%new
    \cite{glass2022uavm}                    & Applied parallel Transformer models are used on top of feature extractors. The proposed method consists of a single model that jointly learns from audio and visual data. This is achieved through a Transformer with shared weights for both modalities (AV) in order to create a shared representation space.\\%new
    \hline
    \cite{rouditchenko2020avlnet}           & Applied parallel projectors to encoder both modalities and ranking losses between representations. \\
    \cite{afouras2021self}                  & Applied co/cross-attention between audio and visual data to generate visual attention maps, which are used to pretrain image object detectors.\\
    \cite{pretet2021cross}                  & Applied Triplet loss for maximizing semantic correlation (i.e., labels) between samples of different modalities. \\
    \cite{zheng2021adversarial}             & Applied Adversarial learning to learn modality-independent features. Semantic information is added through ranking losses (metric learning).\\
    \cite{zeng2020deep}                     & Applied Cluster-CCA and Triplet Loss to maximize correlation between audio and visual data. \\
    \cite{merkx2019language}                & Applied Self-Attention (LSTM) in speech to learn meaningful latent spaces. The authors proposed to learn a joint space between text and images using distance-based loss functions using representations from parallel projections.\\
    \cite{ilharco2019large}                 & Applied parallel projectors using speech and image and maximized their correlation using the cross-covariance matrix. \\
    \cite{he2019new}                        & Applied ranking losses with a shared encoder for 4 modalities. The representation space was constrained using the Center Loss, Classification using supervised information, and ranking losses (QL).\\
    \cite{horiguchi2018face}                & Applied parallel projectors for audio and visual data. Both modalities were correlated using the N-Pair Loss function.\\
    \cite{wu2019unified}                    & Applied self-supervised frameworks for alignment between captions and images to perform text-to-image retrieval. The model consists in co/cross-attention between captions and image locations at different locations.\\
    \cite{cao2016correlation}               & Applied parallel \acrshort*{ae}s and correlates modalities by maximizing correlation in a ``layer-by-layer'' (in the decoder and encoder).\\
    \cite{zhen2019deep}                     & Applied parallel projectors and applied Corr. L. and classification-based loss terms to improve correlation and discrimination in both modalities. \\
    \cite{zhang2021variational}             & Applied a similar approach as the one on \cite{zhen2019deep}, but replaced the projectors with \acrshort*{vae}s.\\
    \cite{zeng2021learning}                 & Applied parallel projectors and trained them to learn unimodal spaces. Both modalities were fused using a linear CCA layer which imposed maximum correlation.\\
    \hline
    \cite{chen2021localizing}               & Applied co/cross-attention between audio and visual data to produce visual attention maps for different instruments. The authors studied the impact of hard negative mining for sound localization. \\
    \cite{lin2020audiovisual}               & Applied co/cross-attention between audio and visual data to produce visual attention maps. The authors explored inter and intra-frame correlations using attention to improve localization performance.\\
    \cite{morgado2020learning}              & Applied parallel reconstructions using the Transformer architecture for video-to-audio and audio-to-video feature translation. The authors trained the model using contrastive losses.\\
    \cite{ramaswamy2020see}                 & Applied parallel attention-based models to produce visual attention maps using attention. The model was trained to synchronize feature representations by leveraging inter-segment (1 seg.) dynamics in videos.\\
    \cite{duan2021audio}                    & Applied co/cross-attention between audio and visual data for event localization tasks. The model was trained for classification.\\
    \hline
    \cite{lin2021exploiting}                & Applied \acrshort*{ae}s to reconstruct bi-aural representations of mono audio. The reconstructions were made using a U-Net model, where its latent spaces are conditioned using visual attention. In other words, the reconstruction was conditioned using an additional loss term which compared visual regions in the image, i.e. different people in different locations in the video frame sequence play different instruments and produce different sounds.\\
    \cite{gao2018learning}                  & Applied Non-Maximum Suppression on attention maps to select the active speaker. Non-Negative Matrix Factorization is used to obtain basis vectors for all audio segments, considered as a "bag" of audio concepts. ImageNet predictions are considered weak labels to train the network.\\%new
    \cite{hu2021dmman}                      & Applied \acrshort*{ae}s generate separate audios given a mixed audio stream and separate visual inputs.\\%new
    \cite{zhu2020visually}                  & Applied an attention-based model for sound separation from a mixed audio stream. Co/cross-attention was computed between different video streams and the same mixed audio clip.\\
    \cite{gao2019co}                        & Applied a U-Net model to separate multiple sound sources in the same audio stream. The reconstructed output was conditioned through concatenation of the U-Net latent space and visual embeddings extracted from \acrshort*{soa} feature extractors.\\
    \cite{zhao2019sound}                    & Similar approach to \cite{gao2019co}, but also considered reconstruction of the video stream and motion trajectories.\\
    \hline
    \cite{hu2020curriculum}                 & Applied parallel feature extractors for both modalities and clusters the reshaped feature maps to find different sound sources and objects.\\
    \cite{zhao2018sound}                    & Applied reconstruction of audio streams using a U-Net model. The Co/cross-attention between the reconstructed spectrograms and visual features were used to separate different sounds.\\%new
    \cite{zhu2021leveraging}                & Similar approach as the one presented in \cite{hu2021dmman}, but consists in parallel projectors instead of using the U-Net model. Additionally, the authors explored how the category of each source can be exploited in sound separation.\\
    \cite{owens2022mix}                     & The model learns representations for separating and localizing sounds through random walks. The authors optimize a sound location model using a dual-stream approach and visual attention. The model is optimized using infoNCE loss. However, they also interpret the attention matrix as a transition matrix between a transition between audio to image. It is used to associate audio embeddings to images by assuming that there exists a one-to-one correspondence between images and sounds. This is similar to the disentanglement learning process (simCLR).\\
    \cite{afouras2020self}                  & Applied visual attention maps integrated over time to find the spatial windows of different objects. Those visual descriptors are used to select the active speaker and separate sound sources.\\%new
    \cite{kanazawa2021choreographer}        & Applied hierarchical attention between Transformer encoders through concatenation and generated future motion given music and motion sequences (auto-regressive approach).\\%new
    \cite{tian2018audio}                    & Applied co/cross-attention between audio and visual data together with metric learning.\\%new
    \hline
\end{longtable}
}


==> tables/applications-table2.tex <==
\begin{table}[]
\centering
\caption{Overview of specific application scenarios of representative works for audio-visual correlation learning}
\label{tab:applications-final}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llll}
\hline
\multicolumn{1}{c}{Paper} & \multicolumn{1}{c}{Main Task} & \multicolumn{1}{c}{Specific Task} & Contribution \\ \hline
\cite{fanzeres2021sound} & Generation & Sound-2-Image Generation & Condition the discriminator using a latent space obtained from reconstruction. \\
\textbf{\cite{zhu2021learning}} & \textbf{Generation} & Cross-Modal (AV) Generation & Multimodal VAE with shared decoder and Wasserstein loss as regularization. \\
\cite{mira2021end} & Generation & Video-2-Speech Generation & Loss considers different aspects of spectrograms (e.g., power, frequency and perceptual quality). \\
\textbf{\cite{gan2020foley}} & \textbf{Generation} & Music Generation & Transformers to translate musing playing visual dynamics (using keypoints) and MIDI output (music). \\
\cite{athanasiadis2020audio} & Generation & Audio \& Video Generation & AEs to map facial crops and speech, which were used as generator in a GAN model for heterogeneity min. between audio and image. \\
\cite{rajan2021robust} & Recognition & Emotion Recognition & \\
\cite{seo2020hmtl} & Recognition & Emotion Recognition &  \\
\cite{zhang2019deep} & Recognition & Emotion Recognition &  \\
\textbf{\cite{recasens2021broaden}} & \textbf{Recognition} & Action Recognition/Sound Classification & \\
\textbf{\cite{ma2020active}} & \textbf{Recognition} & Action Recognition/Sound Classification & \\
\cite{min2021cross} & Recognition & Action Recognition/Sound Classification &  \\
\textbf{\cite{akbari2021vatt}} & \textbf{Recognition} & Action Recognition/Sound Classification & Obtained common representation spaces for video-audio and text-video. \\
\cite{cheng2020look} & Recognition & Action Recognition & \\
\textbf{\cite{patrick2020multi}} & \textbf{Recognition} & Action Recognition/Sound Classification &  \\
\textbf{\cite{MMVAudioSet}} & \textbf{Recognition} & Action Recognition/Sound Classification &  \\
\textbf{\cite{rouditchenko2020avlnet}} & \textbf{Retrieval} & Text-2-Video Retrieval &  \\
\textbf{\cite{afouras2021self}} & \textbf{Retrieval} & Cross-Modal (AV) Retrieval &  \\
\cite{pretet2021cross} & Retrieval & Cross-Modal (AV) Retrieval &  \\
\cite{zheng2021adversarial} & Retrieval & Cross-Modal (AV) Retrieval &  \\
\cite{zeng2020deep} & Retrieval & Cross-Modal (AV) Retrieval & \\
\cite{merkx2019language} & Retrieval & Speech-2-Image Retrieval &  \\
\cite{ilharco2019large} & Retrieval & Cross-Modal (AV) Retrieval &  \\
\cite{he2019new} & Retrieval & Cross-Modal (AVT) Retrieval &  \\
\textbf{\cite{wu2019unified}} & \textbf{Retrieval} & Text-2-Image Retrieval &  \\
\textbf{\cite{cao2016correlation}} & \textbf{Retrieval} & Cross-Modal (IT) Retrieval &  \\
\textbf{\cite{zhang2021variational}} & \textbf{Retrieval} & Cross-Modal (AV) Retrieval &  \\
\textbf{\cite{zhen2019deep}} & \textbf{Retrieval} & Cross-Modal (IT) Retrieval &  \\
\cite{zeng2021learning} & Retrieval & Cross-Modal (AV) Retrieval &  \\
\cite{chen2021localizing} & S. Local. & - &  \\
\textbf{\cite{lin2020audiovisual}} & \textbf{S. Local.} & - &  \\
\textbf{\cite{morgado2020learning}} & \textbf{S. Local.} & - &  \\
\textbf{\cite{ramaswamy2020see}} & \textbf{S. Local.} & - &  \\
\cite{duan2021audio} & S. Local. & - &  \\
\cite{lin2021exploiting} & S. Sep. & - &  \\
\cite{zhu2020visually} & S. Sep. & - &  \\
\textbf{\cite{gao2019co}} & \textbf{S. Sep.} & - &  \\
\textbf{\cite{zhao2019sound}} & \textbf{S. Sep.} & - &  \\
\textbf{\cite{zhu2021leveraging}} & S. Sep. \& Local. & - &  \\
\cite{hu2020curriculum} & S. Sep. \& Local. & - &  \\ \hline
\end{tabular}
}
\end{table}

==> tables/datasets_table.tex <==
\begin{landscape}
\begin{longtable}{@{}p{1.5cm}p{2cm}p{3cm}p{1cm}p{1cm}p{1cm}p{7.5cm}p{7.5cm}@{}}
\caption{Audio-Visual Datasets for Correlation Learning} 
\label{tab:datasets} \\
\hline
Name & Category & Target Task & Env. & Classes & \# clips & Description \\
\hline
%\endfirsthead
%
\endhead
%
%\hline
%\endfoot
%
%\endlastfoot
%
ENST-Drums & Music & Event Rec. & Lab & 10 & 456 & 8 Audio Channels; 2 Video Channels; 720x576; Multiple Classes of music genres; Temporal annotation for each drum event (10 classes); \\
ACAV100M & Real Event & Repres. Lear. & Wild & - & 100M & Clips with 10s at 360p; Multiple sound sources might appear; Automatically curated; High audio-visual correspondence; \\
VGG-SS & Real Event & AV Localization & Wild & 220 & 5158 & Based on VGG-Sounds; sound sources visible in each video clip are explicitly marked with bounding box annotations; \\
ACIVW & Real Event & Repres. Lear. & Wild & 10 & 21000 & Multimodal dataset which provides synchronized data belonging to 3 modalities: acoustic images, audio and RGB frames; Audio and Video are aligned not only in time but also in space; Information can be distilled into monaural audio and audio-visual representations; \\
Countix & Real Event & Video Repetition Counting & Wild & 100 & 8757 & Timecode annotation for the repetitions and the kinetics action class; \\
Kinetics 700-2020 & Real Event & Video Action Rec. & Wild & 700 & 647907 & Multiple sound sources might appear; Sound might not be related with the action occurring in the video; $\sim$10s clips; \\
LLP & Real Event & AV Localization & Wild & 25 & 11849 & Each sound source is annotated; Minimum of 1s per clip; Test set only contains temporal localization of sounds; Each event in the video track is annotated; 10s clips; Overlapping events; \\
VGG Sound & Real Event & Audio-Video Matching & Wild & 309 & 199196 & 10s clips; Audio and video is always semantically correlated (manual verification); Audio-visual correspondent dataset consisting of short clips of audio sounds, extracted from videos uploaded to YouTube; \\
Youtube-ASME-300K & Real Event & Spatial Correspondence & Wild & - & 33725 & 360º videos; 10s clips; ambisonic audio; multiple sound sources in motion; ASMR videos collected from YouTube that contains stereo audio; \\
MEAD & Speech & Emotion Rec. & Lab & 8+7 & 281400 & 1080p at 30 fps clips;  Multi-view data; Emotion and intensity annotations for each speech; Audio and video is paired using a 1s temporal window; \\
FAIR-Play & Music & AV Source Separation & Lab & - & 1871 & Variety of spatial contexts; Biaural recording; 10s clips; The video clip and binaural clip of the same index are roughly aligned; The goal is to convert single channel soundtrack into dual channel by injecting visual information; \\
AVIA & Real Event & AV Localization & Lab & 14 & 378 & Sequences between 30 and 60s; Varying noise conditions for each class; The provided visual and acoustic images are both aligned in space and synchronized in time; \\
CrossTask & Real Event & Video Event Rec. & Wild & 83 & 4700 & The dataset is divided in two parts: 18 primary and 65 related tasks. Videos for the primary tasks are collected manually and provided with annotations for temporal step boundaries. Videos for the related tasks are collected automatically and don't have annotations; Large videos with average length of 4m57s; \\
HowTo100M & Real Event & Video-Language RL & Wild & - & 136M & Narrated audio; 6.5min full clips; After parsing, 4s clips and 4 words; \\
AVA-ActiveSpeaker & Speech & Speaker Detection & Wild & 3 & 38500 & Frame-level annotations; Video track contains the location of each face and active speaker annotations; Audio track contains temporal and categorical annotations for active speaker detection; Missed face tracks can occur; Overlapping active speakers can occur; \\
SEWA & Speech & Human-Activity Underst. & Lab & - & 1990 & 10-30s clips; audio-visual recordings of spontaneous behaviour of volunteers, captured in completely unconstrained, real-world, environments using standard web-cameras and microphones; Audio-visual recordings in the SEWA DB are richly annotated in terms of FAUs, facial landmarks, vocal and verbal cues as well as continuously valued emotion dimensions such as valence, arousal, liking and social signals including agreement and mimicry; \\
MUSIC & Music & AV Source Separation & Lab & 11 & 685 & Clean audio-visual syncronized recordings; Each audio sample is 6s long; \\
MV-10K & Music & AV Retrieval & Wild & - & 10000 & 213-219s clips; "chunks" of 3s; \\
AVA Actions & Real Event & Human-Activity Underst. & Wild & 80 & 430 & Multiple labels per person occurring frequently; Spatio-temporal annotations; Videos from movies; Each 15-min clip is then partitioned into 897 overlapping 3s movie segments with a stride of 1 second; \\
AVE & Real Event & AV Localization & Wild & 28 & 4143 & Multiple sound sources might appear; Test set only contains temporal localization of sounds; 10s clips; Temporal boundary annotations; \\
EPIC-Kitchens & Real Event & Event Rec. & Wild & 149 & 39594 & First person point of view actions in kitchen environments; Temporal annotation for each action; Overlapping actions can appear; Contains object bounding boxes; \\
Moments in Time & Real Event & Event Underst. & Wild & 339 & 791297 & Multiple sound sources might appear; 3s clips; Sourced from a number of different video hosting sites with strong inter \& intra-variations in terms of the number of events depicted in each video. \\
VEGAS & Real Event & Video-Audio Gen. & Wild & 10 & 28109 & $\sim$7s clips; Unbalanced; 10 categories from AudioSet manually curated; \\
AVA-Speech & Speech & Speaker Detection & Wild & 4 & 40000 & Audio track contains temporal and categorical annotations for speech detection; Overlapping active speakers can occur; Categorical labels include background noise; Only the audio track is annotated; \\
AVSpeech & Speech & Speaker Detection & Wild & - & 290000 & Segments of varying length (3-10s); Only one speaker appears;  Collected automatically from Youtube videos; Only contains clean and non-interfering speech; Visual inputs are comprised by only the facial crop and the audio signal; \\
RAVDESS & Speech & AV Vocal Expressions Rec. & Lab & 8+6 & 7356 & 4320 speeches and 3036 songs; created using induced emotional expressions; All conditions are available in three modality formats: Audio-only (16bit, 48kHz .wav), Audio-Video (720p H.264, AAC 48kHz, .mp4), and Video-only (no sound) \\
VoxCeleb2 & Speech & AV Speaker Rec. & Wild & 6112 & 1128246 & $\sim$7.8s clips for each phrase ("utterance"); Audio segments present in the dataset are degraded with background chatter, laughter, overlapping speech and varying room acoustics; \\
C4S & Music & AV Localization & Lab & - & 39000 & 54 videos; The dataset contains labels for the onset, salient points ROIs and the matching sound wave; \\
HIMV-200K & Music & Repres. Lear. & Wild & - & 200500 & Video-music pairs with labels extracted from Youtube-8M (videos labelled as "music video"); \\
URMP & Music & Cross-modal AV Gen. & Lab & 44 & 17555 & 0.5s clip; Image; High quality multi-instrument video dataset recorded in studio and provides ground truth labels for each sound source; For each piece the dataset provided the musical score in MIDI format, the high-quality individual instrument audio recordings and the videos of the assembled pieces; Syncronized; \\
AudioSet & Real Event & Audio Event Rec. & Wild & 485 & 1789621 & 10s clips sampled from 2M videos from youtube; Audio events with the corresponding category and videos; \\
Kinetics-Sounds & Real Event & Video Action Rec. & Wild & 34 & 19000 & Audio and video is not always semantically correlated; 10s clips; Background noise can appear; \\
YouCook2 & Real Event & Procedure Segmentation & Wild & 89 & 2000 & The procedure steps for each video are annotated with temporal boundaries and described by imperative English sentences (see the example below). The videos were downloaded from YouTube and are all in the third-person viewpoint. All the videos are unconstrained and can be performed by individual persons at their houses with unfixed cameras; Average of 7.7 segments per video; \\
LRS & Speech & Lip Reading & Wild & - & 11816 & Metadata contains bounding boxes for each face and spoken sentences; Each sentence is up to 100 characters in length or 10s of duration; Each word has an associated temporal annotation; \\
Flickr-SoundNet & Ambient Sounds & Repres. Lear. & Wild & - & \textgreater{}2M & Unlabeled dataset; Audio-video pairs; \\
MVD & Music & AV Repres. Lear. & Wild & 8 & 2212 & Manual curated dataset; No live performances, abstract or animated videos; Resolution from 320x240 to 640x480; 4m per clip; \\
Charades & Real Event & Audio Event Rec. & Wild & 157 & 9848 & Multiple labels of activities spanning $\sim$30s per clip; Users were presented with a sentence, that includes objects and actions from a fixed vocabulary, and they recorded a video acting out the sentence (charades method); Categorical temporal annotation; \\
MSR-VTT & Real Event & Event Underst. & Wild & 20 & 7180 & Video and sentence pairs; Although the videos are categorized into 20 general categories, the metadata also contains textual descriptions for each video; The duration of each clip is between 10 and 30 seconds; \\
Youtube-8M & Real Event & Video Underst. & Wild & 4800 & 8264650 & Average of 229.6s clips; Each video contains audio and visual modality. Based on the visual information, videos are divided into 24 topics, such as sports, game, arts \& entertainment, etc; \\
LRW & Speech & Lip Reading & Wild & 500 & 1000 & Metadata contains bounding boxes for each face and spoken sentences; Videos are 29 frames (1.16seg); Each word has an associated temporal annotation; \\
ActivityNet & Real Event & Human-Activity Underst. & Wild & 200 & 14950 & Audio and video is not always semantically correlated; Untrimmed activity recognition scenario - predicting ativities in a full video (timecode annotation); Trimmed activity recognition scenario - predict label of a video; In the untrimmed scenario, the videos can contain multiple activities; Diverse and rich taxonomy of activities; \\
ESC-50 & Real Event & Audio Event Classification & Wild & 50 & 2000 & 5-second-long recordings organized into 50 semantical classes (with 40 examples per class) loosely arranged into 5 major categories; \\
Vis. Ind. Sounds & Real Event & Video-Audio Gen. & Wild & 17 & 977 & $\sim$35s clips; Predicting sound from videos as a way to study physical interactions within a visual scene; The dataset contains videos of interations with objects and the matching sounds; \\
OULUVS2 & Speech & Mouth Motion Analysis & Lab & 52 & 3640 & Different points of view;  Utterances: continuous digits, phrases, sentences; \\
TCD-TIMIT & Speech & AV Speech Rec. & Lab & 6913 & 13826 & TCD-TIMIT consists of high-quality audio and video footage of 62 speakers reading a total of 6913 phonetically rich sentences; Video footage was recorded from two angles: straight on, and at 30degrees; \\
UCF-101 & Real Event & Video Action Rec. & Wild & 101 & 13320 & $\sim$7.2s per clip; 320x240px; Dynamic background; Camera motion; Audio and video is not always semantically correlated; \\
HMDB-51 & Real Event & Video Action Rec. & Wild & 51 & 6849 & Video and audio pairs with the associated action category labels; Metadata also contains visible body parts/occlusions, camera motion, camera viewpoint and the number of people involved in the action; \\* \bottomrule
\end{longtable}

\end{landscape}

==> tables/methods-table-v2.tex <==
\begin{landscape}
    \begin{table}
        \centering
        \caption{Overview of representative works for audio-visual correlation learning}
        \label{tab:methods-final}
        \resizebox{1.3\textwidth}{!}{%
            \begin{tabular}{llllllllllll}
                \hline
                \multicolumn{1}{c}{\textbf{Paper}}     & \textbf{P.}         & \textbf{Att.}       & \textbf{AE}         & \textbf{GAN} & \textbf{Loss}          & \textbf{Reg.}                     & \multicolumn{1}{c}{\textbf{Learning}} & \multicolumn{1}{c}{\textbf{Main Task}} & \multicolumn{1}{c}{\textbf{Metrics}} & \textbf{\textbf{Performance}} & \textbf{\textbf{Benchmark Datasets}}  \\ \hline
                \cite{fanzeres2021sound}               & X                   & X                   & \checkmark          & \checkmark   & Adv. Loss              & MSE                               & Self-Sup.                             & Generation                             & I                                    & 0.14                          & VEGAS                                 \\
                \textbf{\cite{zhu2021learning}}        & \textbf{X}          & \textbf{X}          & \textbf{\checkmark} & \textbf{X}   & \textbf{ELBO}          & \textbf{Wasserstein}              & \textbf{UnSup.}                       & \textbf{Generation}                    & \textbf{MRR}                         & \textbf{0.175}                & \textbf{AVE}                          \\
                \cite{mira2021end}                     & X                   & X                   & X                   & \checkmark   & Adv. Loss              & Mult. Discrim.                    & UnSup.                                & Generation                             & WER                                  & 23.13 | 42.51                 & GRID | LRW                            \\
                \textbf{\cite{gan2020foley}}           & \textbf{X}          & \textbf{\checkmark} & \textbf{X}          & \textbf{X}   & \textbf{CE}            & \textbf{-}                        & \textbf{Sup.}                         & \textbf{Generation}                    & \textbf{NDB}                         & \textbf{20}                   & \textbf{MUSIC}                        \\
                \cite{athanasiadis2020audio}           & X                   & X                   & X                   & \checkmark   & Adv. Loss              & Gauss. Noise + CE                 & UnSup.                                & Generation                             & FID                                  & 49.8 / 59.4                   & CREMA-D/RAVDESS                       \\
                \cite{rajan2021robust}                 & X                   & X                   & \checkmark          & X            & MSE                    & CCA + CE                          & Sup.                                  & Recognition                            & ACC                                  & 56.5(A)/55.2(V)               & SEW                                   \\
                \cite{seo2020hmtl}                     & X                   & \checkmark          & X                   & \checkmark   & Adv. Loss              & CE                                & Self-Sup.                             & Recognition                            & ACC                                  & 65.2/40.1                     & CMU-MOSI/IEMOCAP                      \\
                \cite{zhang2019deep}                   & X                   & \checkmark          & X                   & X            & CE                     & -                                 & Sup.                                  & Recognition                            & ACC                                  & 62.5                          & AFEW8.0                               \\
                \textbf{\cite{recasens2021broaden}}    & \textbf{X}          & \textbf{X}          & \textbf{\checkmark} & \textbf{X}   & \textbf{L2}            & \textbf{-}                        & \textbf{Self-Sup.}                    & \textbf{Recognition}                   & \textbf{ACC}                         & \textbf{93.2/69.9/93.}        & \textbf{UCF101/HMDB51/ESC-50}         \\
                \textbf{\cite{ma2020active}}           & \textbf{\checkmark} & \textbf{X}          & \textbf{X}          & \textbf{X}   & \textbf{NCE}           & \textbf{Act. neg. sampl.}         & \textbf{Self-Sup.}                    & \textbf{Recognition}                   & \textbf{ACC}                         & \textbf{94.1/67.2/90.8}       & \textbf{UCF101/HMDB51/ESC-50}         \\
                \cite{min2021cross}                    & X                   & \checkmark          & X                   & X            & NCE                    & L2 (Att. consist.)                & Self-Sup.                             & Recognition                            & ACC                                  & 90.3/61.1/81.4                & UCF101/HMDB51/ESC-50                  \\
                \textbf{\cite{akbari2021vatt}}         & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{X}          & \textbf{X}   & \textbf{MIL-NCE}       & \textbf{-}                        & \textbf{Self-Sup.}                    & \textbf{Recognition}                   & \textbf{ACC}                         & \textbf{89.6/65.2/84.7}       & \textbf{UCF101/HMDB51/ESC-50}         \\
                \cite{cheng2020look}                   & \checkmark          & \checkmark          & X                   & X            & CE                     & -                                 & Self-Sup.                             & Recognition                            & ACC                                  & 87.8/58.2                     & UCF101/HMDB51                         \\
                \textbf{\cite{patrick2020multi}}       & \textbf{\checkmark} & \textbf{X}          & \textbf{X}          & \textbf{X}   & \textbf{NCE}           & \textbf{-}                        & \textbf{Self-Sup.}                    & \textbf{Recognition}                   & \textbf{ACC}                         & \textbf{88.5/95.2/72.8}       & \textbf{ESC-50/UCF101/HMDB51}         \\
                \textbf{\cite{MMVAudioSet}}            & \textbf{\checkmark} & \textbf{X}          & \textbf{X}          & \textbf{X}   & \textbf{MIL-NCE + NCE} & \textbf{-}                        & \textbf{Self-Sup.}                    & \textbf{Recognition}                   & \textbf{ACC}                         & \textbf{88.9/91.8/67.1}       & \textbf{ESC-50/UCF101/HMDB51}         \\
                \textbf{\cite{rouditchenko2020avlnet}} & \textbf{X}          & \textbf{\checkmark} & \textbf{X}          & \textbf{X}   & \textbf{MMS}           & \textbf{-}                        & \textbf{Self-Sup.}                    & \textbf{Retrieval}                     & \textbf{Recall @10}                  & \textbf{49.9/67.9}            & \textbf{MSR-VTT/YouCook2}             \\
                \textbf{\cite{afouras2021self}}        & \textbf{\checkmark} & \textbf{X}          & \textbf{X}          & \textbf{X}   & \textbf{NCE + CE}      & \textbf{-}                        & \textbf{Sup.}                         & \textbf{Retrieval}                     & \textbf{mAP @50}                     & \textbf{39.4/28.}             & \textbf{VGG Sound/AudioSet}           \\
                \cite{pretet2021cross}                 & \checkmark          & X                   & X                   & X            & T                      & -                                 & Self-Sup.                             & Retrieval                              & Recall @10                           & 7.425                         & MVD                                   \\
                \cite{zheng2021adversarial}            & \checkmark          & X                   & X                   & \checkmark   & LSL + Adv. Loss        & -                                 & Sup.                                  & Retrieval                              & ACC                                  & 93                            & VGGFace + VoxCeleb                    \\
                \cite{zeng2020deep}                    & \checkmark          & X                   & X                   & X            & T                      & CCA (feat. align.)                & Sup.                                  & Retrieval                              & mAP                                  & 74.2                          & VEGAS                                 \\
                \cite{merkx2019language}               & \checkmark          & \checkmark          & X                   & X            & Hinge                  & -                                 & Sup.                                  & Retrieval                              & Recall @10                           & 52.3                          & Flikr-8K                              \\
                \cite{ilharco2019large}                & \checkmark          & \checkmark          & X                   & X            & MMS/T                  & -                                 & Sup.                                  & Retrieval                              & Recall @10                           & 52.65                         & Flickr Audio Caption Corpus           \\
                \cite{he2019new}                       & X                   & X                   & X                   & X            & CE                     & Center + QL                       & Sup.                                  & Retrieval                              & mAP                                  & 41.2                          & CUB-200-2011 + Youtube Birds          \\
                \cite{horiguchi2018face}               & \checkmark          & X                   & X                   & X            & NPL                    & -                                 & UnSup.                                & Retrieval                              & mAP                                  & 2.07                          & FVceleb                               \\
                \textbf{\cite{wu2019unified}}          & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{X}          & \textbf{X}   & \textbf{L2}            & \textbf{L1}                       & \textbf{Sup.}                         & \textbf{Retrieval}                     & \textbf{Recall @10}                  & \textbf{71.9}                 & \textbf{MS-COCO}                      \\
                \textbf{\cite{cao2016correlation}}     & \textbf{X}          & \textbf{X}          & \textbf{\checkmark} & \textbf{X}   & \textbf{L2}            & \textbf{L2}                       & \textbf{Sup.}                         & \textbf{Retrieval}                     & \textbf{mAP}                         & \textbf{35.5/71.7}            & \textbf{Wiki Dataset/Flickr}          \\
                \textbf{\cite{zhang2021variational}}   & \textbf{X}          & \textbf{X}          & \textbf{\checkmark} & \textbf{X}   & \textbf{ELBO}          & \textbf{Corr. (CE) + Center + L2} & \textbf{Sup.}                         & \textbf{Retrieval}                     & \textbf{mAP}                         & \textbf{81.2/35.}             & \textbf{VEGAS/AVE}                    \\
                \textbf{\cite{zhen2019deep}}           & \textbf{\checkmark} & \textbf{X}          & \textbf{X}          & \textbf{X}   & \textbf{CE}            & \textbf{Corr. (CE) + L2}          & \textbf{Sup.}                         & \textbf{Retrieval}                     & \textbf{mAP}                         & \textbf{71.6/61.3}            & \textbf{Pascal Sentence/NUS-WIDE-10k} \\
                \cite{zeng2021learning}                & \checkmark          & X                   & X                   & X            & Corr. (DCCA)           & L2 + Frob. Norm                   & Sup.                                  & Retrieval                              & mAP                                  & 77.8/30.8                     & VEGAS/AVE                             \\
                \cite{chen2021localizing}              & \checkmark          & \checkmark          & X                   & X            & NCE                    & -                                 & Self-Sup.                             & S. Local.                              & AUC                                  & 0.573/0.590                   & Flickr-SoundNet/VGG-SS                \\
                \textbf{\cite{lin2020audiovisual}}     & \textbf{X}          & \textbf{\checkmark} & \textbf{X}          & \textbf{X}   & \textbf{CE}            & \textbf{-}                        & \textbf{Self-Sup.}                    & \textbf{S. Local.}                     & \textbf{ACC}                         & \textbf{76.8}                 & \textbf{AVE}                          \\
                \textbf{\cite{morgado2020learning}}    & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{X}          & \textbf{X}   & \textbf{NCE}           & \textbf{-}                        & \textbf{Self-Sup.}                    & \textbf{S. Local.}                     & \textbf{ACC}                         & \textbf{73.85/73.8/37.66}     & \textbf{YT-360/UCF-101/HMDB51}        \\
                \textbf{\cite{ramaswamy2020see}}       & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{X}          & \textbf{X}   & \textbf{CE/T}          & \textbf{-}                        & \textbf{Self-/(Un)Sup.}               & \textbf{S. Local.}                     & \textbf{ACC}                         & \textbf{74.8}                 & \textbf{AVE}                          \\
                \cite{duan2021audio}                   & \checkmark          & \checkmark          & X                   & X            & CE                     & -                                 & Sup.                                  & S. Local.                              & ACC                                  & 76.2                          & AVE                                   \\
                \cite{lin2021exploiting}               & X                   & \checkmark          & \checkmark          & X            & CE + L2                & -                                 & Self-Sup.                             & S. Sep.                                & STFT                                 & 0.865/1.448                   & FAIR PLAY/YT-MUSIC                    \\
                \cite{zhu2020visually}                 & \checkmark          & \checkmark          & X                   & X            & CE                     & -                                 & Sup.                                  & S. Sep.                                & SDR                                  & 8.25                          & MUSIC                                 \\
                \textbf{\cite{gao2019co}}              & \textbf{X}          & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{X}   & \textbf{L1 + CE}       & \textbf{-}                        & \textbf{Sup.}                         & \textbf{S. Sep.}                       & \textbf{SDR}                         & \textbf{7.64}                 & \textbf{MUSIC}                        \\
                \textbf{\cite{zhao2019sound}}          & \textbf{X}          & \textbf{\checkmark} & \textbf{\checkmark} & \textbf{X}   & \textbf{CE}            & \textbf{-}                        & \textbf{Self-Sup.}                    & \textbf{S. Sep.}                       & \textbf{SDR}                         & \textbf{8.31}                 & \textbf{MUSIC}                        \\
                \cite{zhu2021leveraging}               & \checkmark          & \checkmark          & X                   & X            & CE                     & -                                 & Self-Sup.                             & S. Sep. \& Local.                      & SDR                                  & 10.74                         & MUSIC                                 \\
                \cite{hu2020curriculum}                & X                   & \checkmark          & \checkmark          & X            & CL + L1 (S. Sep.)      & -                                 & Self-Sup.                             & S. Sep. \& Local.                      & AUC/SDR                              & 49.2/6.59                     & Flickr-SoundNet/MUSIC                 \\ \hline
            \end{tabular}%
        }
    \end{table}
\end{landscape}
